Revisiting Deep Audio-Text Retrieval Through the Lens of Transportation

The Learning-to-match (LTM) framework proves to be an effective inverse optimal transport approach for learning the underlying ground metric between two sources of data, facilitating subsequent matching. However, the conventional LTM framework faces scalability challenges, necessitating the use of the entire dataset each time the parameters of the ground metric are updated. In adapting LTM to the deep learning context, we introduce the mini-batch Learning-to-match (m-LTM) framework for audio-text retrieval problems. This framework leverages mini-batch subsampling and Mahalanobis-enhanced family of ground metrics. Moreover, to cope with misaligned training data in practice, we propose a variant using partial optimal transport to mitigate the harm of misaligned data pairs in training data. We conduct extensive experiments on audio-text matching problems using three datasets: AudioCaps, Clotho, and ESC-50. Results demonstrate that our proposed method is capable of learning rich and expressive joint embedding space, which achieves SOTA performance. Beyond this, the proposed m-LTM framework is able to close the modality gap across audio and text embedding, which surpasses both triplet and contrastive loss in the zero-shot sound event detection task on the ESC-50 dataset. Notably, our strategy of employing partial optimal transport with m-LTM demonstrates greater noise tolerance than contrastive loss, especially under varying noise ratios in training data on the AudioCaps dataset. Our code is available at https://github.com/v-manhlt3/m-LTM-Audio-Text-Retrieval

==> latex-folder/2.3.tex <==
Denote $\{x_i,y_i\}_{i=1}^n$ is all pairs of audio and caption in the training dataset, the goal is to learn an energy model to define the joint probability between audio and text:
\begin{equation}
\label{eq:6}
    \begin{aligned}
    & p(X,Y) = \frac{\exp(-E_{\psi}(X,Y))}{Z(\psi)} \text{, where } Z(\psi) = \int\int\exp(-E_{\psi}(X,Y))dXdY
    \end{aligned}
\end{equation}
, the energy function $E_{\psi}(.)$ is parameterized by $\psi=\{\theta, \phi\}$ which implicitly consists of two encoders, audio encoder $f_{\theta}(x)$ and text encoder $g_{\phi}(y)$. Given two fixed encoders, the energy function between two modalities is defined as the cosine similarity function $E_{\theta,\phi}(x,y)=\frac{<f_{\theta}(x).g_{\phi}(y)>}{||f_{\theta}(x)||_2||g_{\phi}(y)||_2}$. During training, only a minibatch of data $(X^b,Y^b)=\{x_i,y_i\}_{i=1}^b$ is sampled to train the energy function $E_{\theta,\phi}(.)$ by maximizing the cross-entropy objective function:
\begin{equation}
\begin{aligned}
    H(\tilde{p}|p_{\theta,\phi}) &= \mathbb{E}_{(X^b,Y^b) \sim D} \big[\tilde{p}(X^b,Y^b)\log(p_{\theta,\phi}(X^b,Y^b))\big] \\
    &=\mathbb{E}_{(X^b,Y^b) \sim D}[\sum_{i=1}^b\sum_{j=1}^b \tilde{p}(x_i,y_i)\log{p_{\theta,\phi}(x_i,y_i)}]\\
\end{aligned}
\end{equation}
, where $\tilde{p}(X^b,Y^b)$ is a diagonal matrix whose diagonal is $\frac{1}{b}$ and $p_{\theta, \phi}(X^b,Y^b)$ is the matrix of joint probability defined by the energy function.

At the inference stage, given $n$ audio $\{x_i\}_{i=1}^n$ and $m$ caption $\{y_j\}_{j=1}^m$, the ranking matrix $P(\{x_i\}_{i=1}^n, \{y_j\}_{j=1}^m)$ between two sets of audio and caption can be retrieved by utilizing the learned energy function. For example, the correspondence caption of a given audio $x_i$ is
\begin{equation}
\label{eq:7}
    \hat{y} = \argmax_y \frac{\exp(-E_{\theta,\phi}(x_i, y))}{\sum_{j=1}^m\exp(-E_{\theta,\phi}(x_i,y_j))}
\end{equation}

==> latex-folder/4.2-old.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=1\textwidth]{ICLR-2024/Fig/Noisy-Corres.pdf}
%     \caption{The visualization of ideal minibatch matching from Partial OT with different values of total transportation mass($m$) and the contrastive learning. The minibatch target matching is an incomplete matching with no matching for the first row. The ideal matching from contrastive learning fails to take the incomplete matching into account, while Partial OT can recover the incomplete matching with appropriate transportation mass($m=\frac{2}{3}$) }
%     \label{fig:1}
% \end{figure*}a

\textcolor{blue}{a Manh should separate this section in two multiple paragraphs: \textbf{Noisy correspondence setting} (only explain the construction of the noisy and why should we care about this setting in practice and cite something), \textbf{Mini-batch learning to match under noisy correspondence setting} (write the objective, explain why it is suck), \textbf{Mini-batch partial learning to match.} Write the definition of POT, and the objective, and explain why it is better. }

\textbf{Noisy correspondence setting.} We first introduce the noisy correspondence setting for the audio-text matching task. That is, given the training data $D=\{(x_i,y_i)\}_{i=1}^N$ where $N$ is the number of training samples, a proportion of training data $N_{cor}$, $N_{cor}<N$, is corrupted, for instance, due to the data collection process. The amount of data corruption is unknown, and we do not know which samples are corrupt, thus presenting a challenging learning scenario.

% Due to the noisy correspondence phenomenon, the true matching $\pi^*$ is now corrupted to an incomplete matching $\bar{\pi}$, in which there is no matching in some rows. The visualization of empirical and incomplete matching within a minibatch is illustrated in Figure.~\ref{fig:1}. We denote a random variable $z \in \{0,1\}$ which is sampled from a binomial distribution $Binomial(N,1-\frac{N_{cor}}{N})$. If $z=1$ indicates the audio-text pair is true matching, otherwise the audio-text pair is wrong matching. The training data is now $\Tilde{D}=\{(z_i, x_i, y_i)\}_{i=1}^N$, where $z_i \sim Binomial(N,1-\frac{N_{cor}}{N})$. Since the data corruption is unknown, we only have the empirical matching $\hat{\pi}$ for training. The final goal is to learn the true matching $\bar{\pi}$ from the noisy training data $\Tilde{D}$. Hence, we propose to use Partial OT to mitigate the harmfulness of noisy empirical matching for approximating the true matching $\bar{\pi}$. As illustrated in Figure.~\ref{fig:1}, the ideal matching from Partial OT with appropriate transportation mass($s=\frac{2}{3}$) can recover the incomplete matching $\bar{\pi}$, while contrastive learning is not able to approximate the incomplete matching. The objective function~\ref{eq:10} is rewritten as 
Due to the noisy correspondence phenomenon, the empirical matching $\hat{\pi}$ is now corrupted to an incomplete matching $\bar{\pi}$, in which there is no matching in some rows. The visualization of empirical and incomplete matching within a minibatch is illustrated in Figure.~\ref{fig:1}. Assuming an absence of noise in the original training data, we introduce noisy correspondence training samples by randomly shuffling a portion of audio-text pairs. We denote a random variable $z \in \{0,1\}$ which is sampled from a binomial distribution $Binomial(N,1-\frac{N_{cor}}{N})$, if $z=1$ indicates the audio-text pair is shuffled. The training data is now $\Tilde{D}=\{(z_i, x_i, y_i)\}_{i=1}^N$, where $z_i \sim Binomial(N,1-\frac{N_{cor}}{N})$. Since the data corruption is unknown, we only have the empirical matching $\hat{\pi}$ for training. The final goal is to learn the true matching $\bar{\pi}$ from the noisy training data $\Tilde{D}$. Hence, we propose to use Partial OT to mitigate the harmfulness of noisy empirical matching for approximating the true matching $\bar{\pi}$. As illustrated in Figure.~\ref{fig:1}, the ideal matching from Partial OT with appropriate transportation mass($s=\frac{2}{3}$) can recover the incomplete matching $\bar{\pi}$, while contrastive learning is not able to approximate the incomplete matching. The objective function~\ref{eq:10} is rewritten as 
\begin{equation}
    \begin{aligned}
        &\underset{\psi}{\min } \underset{(\Tilde{X}^b,\Tilde{Y}^b) \sim \Tilde{D}}{\mathbb{E}} \bigg[\text{KL}(\hat{\pi}^{\Tilde{X^b},\Tilde{Y^b}} ||\pi_{\epsilon, s}^{C(\Tilde{X^b},\Tilde{Y^b};M)} \bigg], \\
    &\text{subject to } M \succeq 0
    \end{aligned}
\end{equation}
, where $(\Tilde{X}^b, \Tilde{Y}^b)$ is a minibatch sampled from noisy training data $\Tilde{D}$, and $\pi_{\epsilon, s}^{\Tilde{X}^b,\Tilde{Y}^b}$ is the optimal solution the equation
\begin{align}
\label{eq:2}
    \pi_{\epsilon, s}^{C(\Tilde{X^b},\Tilde{Y^b};M)}= \underset{\pi \in \Pi_s(u_b,u_b)}{\argmin} \langle C(\Tilde{X}^b, \Tilde{Y}^b;M), \pi \rangle - \epsilon H(\pi),
\end{align}
where $\Pi_s(u_b,u_b)=\{\pi \in \mathbb{R}_+^{n \times m}|\pi \mathds{1} \leq u_b ,\pi^\top \mathds{1} \leq u_b, \mathds{1}\mathbf{\pi}^\top  \mathds{1}=s\}$. The partial OT optimization can be solved by using Bregman projection ~\citep{benamou2015iterative}. Intuitively, the partial transportation plan should be such that true correspondence audio-text pairs within a minibatch are mapped to each other, while noisy correspondence audio-text pairs are discarded from the transportation plan. We conducted an experiment to examine the relationship between the transportation mass and noise ratio in training data in the Section.~\ref{sec:noisy_exp}
% with $\bar{\alpha}=[ \alpha, ||\beta||_1-m ]$ and $\bar{\beta}=[ \beta, ||\alpha||_1-m ]$. Partial OT optimization can be solved by using Bregman projection~\citep{benamou2015iterative}

==> notes/macros.tex <==
\newcommand{\sidenote}[1]{\marginpar{\small \emph{\color{Medium}#1}}}

\global\long\def\se{\hat{\text{se}}}%

\global\long\def\interior{\text{int}}%

\global\long\def\boundary{\text{bd}}%

\global\long\def\ML{\textsf{ML}}%

\global\long\def\GML{\mathsf{GML}}%

\global\long\def\HMM{\mathsf{HMM}}%

\global\long\def\support{\text{supp}}%

\global\long\def\new{\text{*}}%

\global\long\def\stir{\text{Stirl}}%

\global\long\def\mA{\mathcal{A}}%

\global\long\def\mB{\mathcal{B}}%

\global\long\def\mF{\mathcal{F}}%

\global\long\def\mK{\mathcal{K}}%

\global\long\def\mH{\mathcal{H}}%

\global\long\def\mX{\mathcal{X}}%

\global\long\def\mY{\mathcal{Y}}%

\global\long\def\mZ{\mathcal{Z}}%

\global\long\def\mS{\mathcal{S}}%

\global\long\def\Ical{\mathcal{I}}%

\global\long\def\mT{\mathcal{T}}%

\global\long\def\Pcal{\mathcal{P}}%

\global\long\def\dist{d}%

\global\long\def\HX{\entro\left(X\right)}%
 
\global\long\def\entropyX{\HX}%

\global\long\def\HY{\entro\left(Y\right)}%
 
\global\long\def\entropyY{\HY}%

\global\long\def\HXY{\entro\left(X,Y\right)}%
 
\global\long\def\entropyXY{\HXY}%

\global\long\def\mutualXY{\mutual\left(X;Y\right)}%
 
\global\long\def\mutinfoXY{\mutualXY}%

\global\long\def\given{\mid}%

\global\long\def\gv{\given}%

\global\long\def\goto{\rightarrow}%

\global\long\def\asgoto{\stackrel{a.s.}{\longrightarrow}}%

\global\long\def\pgoto{\stackrel{p}{\longrightarrow}}%

\global\long\def\dgoto{\stackrel{d}{\longrightarrow}}%

\global\long\def\lik{\mathcal{L}}%

\global\long\def\logll{\mathit{l}}%

\global\long\def\vectorize#1{\mathbf{#1}}%
 

\global\long\def\vt#1{\mathbf{#1}}%

\global\long\def\gvt#1{\boldsymbol{#1}}%

\global\long\def\idp{\ \bot\negthickspace\negthickspace\bot\ }%
 
\global\long\def\cdp{\idp}%

\global\long\def\das{:=}%

\global\long\def\id{\mathbb{I}}%

\global\long\def\idarg#1#2{\id\left\{  #1,#2\right\}  }%

\global\long\def\iid{\stackrel{\text{iid}}{\sim}}%

\global\long\def\bzero{\vt 0}%

\global\long\def\bone{\mathbf{1}}%

\global\long\def\boldm{\boldsymbol{m}}%

\global\long\def\bff{\vt f}%

\global\long\def\bx{\boldsymbol{x}}%

\global\long\def\ba{\boldsymbol{a}}%

\global\long\def\bb{\boldsymbol{b}}%

\global\long\def\bc{\boldsymbol{c}}%

\global\long\def\bl{\boldsymbol{l}}%

\global\long\def\bu{\boldsymbol{u}}%

\global\long\def\bo{\boldsymbol{o}}%

\global\long\def\bh{\boldsymbol{h}}%

\global\long\def\bs{\boldsymbol{s}}%

\global\long\def\bz{\boldsymbol{z}}%

\global\long\def\xnew{y}%

\global\long\def\bxnew{\boldsymbol{y}}%

\global\long\def\bX{\boldsymbol{X}}%

\global\long\def\tbx{\tilde{\bx}}%

\global\long\def\by{\boldsymbol{y}}%

\global\long\def\bY{\boldsymbol{Y}}%

\global\long\def\bZ{\boldsymbol{Z}}%

\global\long\def\bU{\boldsymbol{U}}%

\global\long\def\bv{\boldsymbol{v}}%

\global\long\def\bn{\boldsymbol{n}}%

\global\long\def\bV{\boldsymbol{V}}%

\global\long\def\bI{\boldsymbol{I}}%

\global\long\def\bw{\vt w}%

\global\long\def\bW{\boldsymbol{W}}%

\global\long\def\balpha{\gvt{\alpha}}%

\global\long\def\bbeta{\gvt{\beta}}%

\global\long\def\bmu{\gvt{\mu}}%

\global\long\def\btheta{\boldsymbol{\theta}}%

\global\long\def\blambda{\boldsymbol{\lambda}}%

\global\long\def\bgamma{\boldsymbol{\gamma}}%

\global\long\def\bpsi{\boldsymbol{\psi}}%

\global\long\def\bphi{\boldsymbol{\phi}}%

\global\long\def\bpi{\boldsymbol{\pi}}%

\global\long\def\bomega{\boldsymbol{\omega}}%

\global\long\def\bepsilon{\boldsymbol{\epsilon}}%

\global\long\def\btau{\boldsymbol{\tau}}%

\global\long\def\bxi{\boldsymbol{\xi}}%

\global\long\def\realset{\mathbb{R}}%

\global\long\def\realn{\realset^{n}}%

\global\long\def\integerset{\mathbb{Z}}%

\global\long\def\natset{\integerset}%

\global\long\def\integer{\integerset}%
 

\global\long\def\natn{\natset^{n}}%

\global\long\def\rational{\mathbb{Q}}%

\global\long\def\rationaln{\rational^{n}}%

\global\long\def\complexset{\mathbb{C}}%

\global\long\def\comp{\complexset}%
 

\global\long\def\compl#1{#1^{\text{c}}}%

\global\long\def\and{\cap}%

\global\long\def\compn{\comp^{n}}%

\global\long\def\comb#1#2{\left({#1\atop #2}\right) }%

\global\long\def\nchoosek#1#2{\left({#1\atop #2}\right)}%

\global\long\def\param{\vt w}%

\global\long\def\Param{\Theta}%

\global\long\def\meanparam{\gvt{\mu}}%

\global\long\def\Meanparam{\mathcal{M}}%

\global\long\def\meanmap{\mathbf{m}}%

\global\long\def\logpart{A}%

\global\long\def\simplex{\Delta}%

\global\long\def\simplexn{\simplex^{n}}%

\global\long\def\dirproc{\text{DP}}%

\global\long\def\ggproc{\text{GG}}%

\global\long\def\DP{\text{DP}}%

\global\long\def\ndp{\text{nDP}}%

\global\long\def\hdp{\text{HDP}}%

\global\long\def\gempdf{\text{GEM}}%

\global\long\def\rfs{\text{RFS}}%

\global\long\def\bernrfs{\text{BernoulliRFS}}%

\global\long\def\poissrfs{\text{PoissonRFS}}%

\global\long\def\iidrfs{$\text{IidRFS}$}%

\global\long\def\grad{\gradient}%
 
\global\long\def\gradient{\nabla}%

\global\long\def\partdev#1#2{\partialdev{#1}{#2}}%
 
\global\long\def\partialdev#1#2{\frac{\partial#1}{\partial#2}}%

\global\long\def\partddev#1#2{\partialdevdev{#1}{#2}}%
 
\global\long\def\partialdevdev#1#2{\frac{\partial^{2}#1}{\partial#2\partial#2^{\top}}}%

\global\long\def\hessian{\text{Hess}}%

\global\long\def\closure{\text{cl}}%

\global\long\def\cpr#1#2{\Pr\left(#1\ |\ #2\right)}%

\global\long\def\var{\text{Var}}%

\global\long\def\Var#1{\text{Var}\left[#1\right]}%

\global\long\def\cov{\text{Cov}}%

\global\long\def\Cov#1{\cov\left[ #1 \right]}%

\global\long\def\COV#1#2{\underset{#2}{\cov}\left[ #1 \right]}%

\global\long\def\corr{\text{Corr}}%

\global\long\def\sst{\text{T}}%

\global\long\def\SST{\sst}%

\global\long\def\ess{\mathbb{E}}%

\global\long\def\Ess#1{\mathbb{E}\left[#1\right]}%

\newcommandx\ESS[2][usedefault, addprefix=\global, 1=]{\underset{#2}{\mathbb{E}}\left[#1\right]}%

\global\long\def\fisher{\mathcal{F}}%
 

\global\long\def\bfield{\mathcal{B}}%
 
\global\long\def\borel{\mathcal{B}}%

\global\long\def\bernpdf{\text{Bernoulli}}%

\global\long\def\betapdf{\text{Beta}}%

\global\long\def\dirpdf{\text{Dir}}%

\global\long\def\gammapdf{\text{Gamma}}%

\global\long\def\gaussden#1#2{\text{Normal}\left(#1, #2 \right) }%

\global\long\def\gauss{\mathbf{N}}%

\global\long\def\gausspdf#1#2#3{\text{Normal}\left( #1 \lcabra{#2, #3}\right) }%

\global\long\def\multpdf{\text{Mult}}%

\global\long\def\poiss{\text{Pois}}%

\global\long\def\poissonpdf{\text{Poisson}}%

\global\long\def\pgpdf{\text{PG}}%

\global\long\def\wshpdf{\text{Wish}}%

\global\long\def\iwshpdf{\text{InvWish}}%

\global\long\def\nwpdf{\text{NW}}%

\global\long\def\niwpdf{\text{NIW}}%

\global\long\def\studentpdf{\text{Student}}%

\global\long\def\unipdf{\text{Uni}}%

\global\long\def\transp#1{\transpose{#1}}%
 
\global\long\def\transpose#1{#1^{\mathsf{T}}}%

\global\long\def\mgt{\succ}%

\global\long\def\mge{\succeq}%

\global\long\def\idenmat{\mathbf{I}}%

\global\long\def\trace{\mathrm{tr}}%

\global\long\def\argmax#1{\underset{_{#1}}{\text{argmax}} }%

\global\long\def\argmin#1{\underset{_{#1}}{\text{argmin}\ } }%

\global\long\def\diag{\text{diag}}%

\global\long\def\norm{}%

\global\long\def\spn{\text{span}}%

\global\long\def\vtspace{\mathcal{V}}%

\global\long\def\field{\mathcal{F}}%
 
\global\long\def\ffield{\mathcal{F}}%

\global\long\def\inner#1#2{\left\langle #1,#2\right\rangle }%
 
\global\long\def\iprod#1#2{\inner{#1}{#2}}%

\global\long\def\dprod#1#2{#1 \cdot#2}%

\global\long\def\norm#1{\left\Vert #1\right\Vert }%

\global\long\def\entro{\mathbb{H}}%

\global\long\def\entropy{\mathbb{H}}%

\global\long\def\Entro#1{\entro\left[#1\right]}%

\global\long\def\Entropy#1{\Entro{#1}}%

\global\long\def\mutinfo{\mathbb{I}}%

\global\long\def\relH{\mathit{D}}%

\global\long\def\reldiv#1#2{\relH\left(#1||#2\right)}%

\global\long\def\KL{KL}%

\global\long\def\KLdiv#1#2{\KL\left(#1\parallel#2\right)}%
 
\global\long\def\KLdivergence#1#2{\KL\left(#1\ \parallel\ #2\right)}%

\global\long\def\crossH{\mathcal{C}}%
 
\global\long\def\crossentropy{\mathcal{C}}%

\global\long\def\crossHxy#1#2{\crossentropy\left(#1\parallel#2\right)}%

\global\long\def\breg{\text{BD}}%

\global\long\def\lcabra#1{\left|#1\right.}%

\global\long\def\lbra#1{\lcabra{#1}}%

\global\long\def\rcabra#1{\left.#1\right|}%

\global\long\def\rbra#1{\rcabra{#1}}%


